RecPipe: Co-designing Models and Hardware to Jointly Optimize Recommendation Quality and Performance

Deep learning recommendation systems must provide high quality, personalized content under strict tail-latency targets and high system loads. This paper presents RecPipe, a system to jointly optimize recommendation quality and inference performance. Central to RecPipe is decomposing recommendation models into multi-stage pipelines to maintain quality while reducing compute complexity and exposing distinct parallelism opportunities. RecPipe implements an inference scheduler to map multi-stage recommendation engines onto commodity, heterogeneous platforms (e.g., CPUs, GPUs).While the hardware-aware scheduling improves ranking efficiency, the commodity platforms suffer from many limitations requiring specialized hardware. Thus, we design RecPipeAccel (RPAccel), a custom accelerator that jointly optimizes quality, tail-latency, and system throughput. RPAc-cel is designed specifically to exploit the distinct design space opened via RecPipe. In particular, RPAccel processes queries in sub-batches to pipeline recommendation stages, implements dual static and dynamic embedding caches, a set of top-k filtering units, and a reconfigurable systolic array. Com-pared to prior-art and at iso-quality, we demonstrate that RPAccel improves latency and throughput by 3x and 6x.

==> text/Intro_backup.tex <==
Recommendation algorithms are widely used to enable high-quality and meaningful interactions, for example, to rank social media posts~\cite{instagramMsr}, search queries~\cite{}, movies and videos~\cite{}, and e-commerce products~\cite{zhou2018deep, zhou2019deep}. 
The ever-increasing performance of systems~\cite{}, coupled with the proliferation of data~\cite{}, have enabled fast evolution of recommendation algorithms in the past decade, from traditional matrix factorization~\cite{}, cluster~\cite{}, and nearest neighbor techniques~\cite{} to deep learning-based approaches~\cite{}. 
In fact, Deep Neural Network (DNN) based recommendation models constitutes over 50\% of all AI training and 80\% of all AI inference cycles in Facebook's data center. Similar demands are found across Internet companies including Google and Alibaba~\cite{tpu, }.
These resource demands will continue to grow as more sophisticated DNN-based recommendation models are deployed~\cite{}.

%Given the increased availability of data over the past ten years, recommendation algorithms have evolved from using traditional matrix factorization, clustering, and nearest neighbor techniques to more sophisticated deep learning-based solutions.

%In fact over 60\% of videos on Netflix and Youtube, and 30\% of items bought on Amazon are attributed to recommendation engines.
%However, DNN-based recommendation models pose heavy system requirements.
%For example, DNN-based recommendation models consume over 80\% of Facebook's AI inference cycles; similar capacity requirements are found in Google and Alibaba's data centers~\cite{tpu,alibaba}.
%Deploying recommendation services pose 
%perform recommendation inference under strict latency targets set by service level agreements (SLAs) while sustaining high throughput to serve potentially billions of users worldwide.

Given the importance of DNN-based recommendation models, domain-specific architecture (DSA) solutions are emerging. 
First, compared to convolutional and recurrent neural networks, DNN-based recommendation models comprise embedding table operations that exhibit highly irregular memory access patterns and large storage capacities~\cite{gupta2020architectural}.
Recent work proposed specialized near-memory processing hardware to accelerate embedding operations central to recommendation~\cite{tensordimm, recnmp}.
In addition to accelerating individual operators, Centaur~\cite{centaur}, a hybrid sparse-dense accelerator, was demonstrated to reduce recommendation inference latency. 
%However, recommendation systems must meet both strict tail-latency targets set by service-level agreements (SLAs) and high system throughput to enable applications that serve billions of users worldwide.
Taking a step further to optimize inference latency-bounded throughput, specialized recommendation query schedulers were proposed to partition work across general purpose CPUs and specialized AI-hardware~\cite{gupta2020deeprecsys}. 

%\textcolor{blue}{[Talk about the related works here, follow by what the remaining gaps are and what's addressed by this work.]}

%accelerated hardware accelerators for 

%llion of parameters that pose high compute requirements, irregular memory access patterns, and storage capacities.



%\textcolor{blue}{Condense into the previous P.} While modern deep-learning solutions improve user experiences through higher quality recommendation, they exacerbate system requirements.
%First, DNN-based recommendation models comprise billions of parameters that pose high compute requirements, irregular memory access patterns, and storage capacities.
%For each input query DNN-based recommendation models rank potentially thousands of items to identify the best, most personalized content.
%The combination of large models and query sizes results in long inference latencies that make meeting strict tail-latency thresholds set by application-level service-level agreements (SLAs) challenging.
%In fact, SLA targets for recommendation systems vary from tens to hundreds of milliseconds posing a diverse range of design challenges~\cite{gupta2020deeprecsys}.
%In addition to meeting strict tail-latency targets, recommendation systems must operate at high throughput owing to applications serving potentially billions of users worldwide.
% Not a fan of this here...
%Thus, efficient deployment of recommendation systems requires judiciously balancing the benefits of more sophisticated recommendation systems (e.g., quality) with the challenges they pose (e.g., latency, throughput).
%recommendation quality of more sophisticated models and the challen resulting latency and system throughput 
%Thus, efficiently deploying recommendation systems requires carefully balancing recommendation quality, latency, and throughput.

%Although the aforementioned architectural innovations optimize individual recommendation models, data center scale systems typically comprise many models that collaboratively rank content.

To-date, DSA accelerators have been designed for monolithic DNN-based models, individually. Instead, this work explores algorithm-architecture co-design opportunities for DNN-based recommendation models by decomposing monolithic models into multi-model systems. 
As depicted in Figure~\ref{fig:overview}(a), \textcolor{blue}{this work is one of the few first ones that approaches system design and optimization by co-designing model architectures and hardware.} 
%By doing so, we optimize recommendation quality, inference tail-latency, and system throughput 
In particular, this work builds upon insights from recent multi-stage modeling approaches to reduce the computational complexity of personalized ranking~\cite{instagram, multitask, gupta2020architectural}. 


Inputs to recommendation systems are a large number of items (in the order of thousands) that are each ranked with complex DNN-based models. Combined with the stringent model quality requirement, recommendation models incur 
%Unfortunately, meeting strict SLA targets while ranking a large number of candidate items with complex DNN-based models incurs 
heavy compute and infrastructure demands.
To reduce the ever-increasing resource requirement, multi-stage systems use a ranking funnel to evaluate candidate items, as shown in Figure~\ref{fig:overview}(b).
From the system's perspective, latency-bounded performance and efficiency can be significantly improved when recommendation systems are decomposed into fine-grained multi-stage execution pipeline.
Figure~\ref{fig:overview}(c) shows significant 5.3$\times$ and 5.9$\times$ memory and compute resource demand reduction when monolithic models are decomposed into multi-stage execution.

%Note that such multi-stage designs are used in YouTube's video recommendation system, Instagram social media platform, and \cite{}.
%Intuitively, earlier stages filter candidate items using light-weight models while later stages are heavier-weight in order to perform fine-grained ranking to identify the most relevant candidate items.
%Compared with models in later stages, light-weight models comprise orders of magnitude lower FLOPs, memory lookups, and memory capacity demands.
%Algorithmically, filtering candidate items using light-weight models can significantly reduce the overall compute and memory demands of recommendation systems. 

%One approach to balancing recommendation quality, latency, and throughput is to use multi-stage recommendation systems~\cite{multitask, instagram, gupta2020architectural}.
%Compared to typical single-stage recommendation systems, multi-stage systems reduce the computational complexity of ranking large sets of candidate items.
%Intuitively,  and reduce overall computational complexity.

\begin{figure}[t!]
  \centering
  \includegraphics[width=\columnwidth]{figures/Overview.pdf}
  \caption{ This work combines recent advances from machine learning and computer architecture researchers in optimizing personalized recommendation systems (Left).
  With fine-grained algorithm-hardware co-design across multi-stage recommendation systems we can optimize quality, inference tail-latency, and system throughput. }
  \label{fig:overview}
  \vspace{-1em}     
\end{figure}


%Multi-stage recommendation provide a unique opportunity for systems designers to trade off individual model accuracy and run-time performance to maximize end to end system quality, latency, and throughput.
%Co-designing algorithm and hardware solutions across the stages widens the design space of system solutions as compared to optimizing each stage individually.
%Multi-stage recommendation systems provide unique system design opportunities to balance recommendation quality, latency, and throughput.

At a high level, each stage in the ranking funnel poses unique performance bottlenecks and acceleration opportunities.
Earlier stages implement light-weight models (e.g., low compute and memory demands) with large input sizes, exhibiting high degrees of data-parallelism opportunities.
On the other hand, later ranking stages implement more sophisticated models with high compute demands (e.g., billions of FLOPs) and memory demands (e.g., many GBs of storage).
As such, ranking models exhibit low data-parallelism opportunities but high model-parallelism opportunities.
These differences require intrinsically different system designs for efficient execution across multi-stage recommendation systems.
In fact, our results demonstrate that, compared with previous state-of-the-arts, designing specialized accelerators that exploit these distinct data-parallelism and model-parallelism opportunities can lead to tail-latency and system-throughput improvement by 3$\times$ and 4$\times$, respectively.


Furthermore, to maximize overall recommendation quality under strict performance and resource constraints, designers must balance the accuracy and performance of individual models.
%Compared to CNNs and RNNs, 
Multi-stage recommendation systems allow rigorous and quantitative trade-offs between model accuracy versus performance using two key design parameters: model complexity and number of candidate items.
Increasing model complexity and increasing the number of candidate items both improve ranking quality while degrading run-time performance.
Given these distinct parameters, our analysis demonstrates that under resource constraints, it is often advantageous to deploy less sophisticated, accurate models with larger candidate items to achieve comparable recommendation quality but with much higher throughput performance.


In this work, we propose a framework that enables design space exploration for hardware-software co-design and optimization, tailored for deep learning recommendation models. The framework is called \Infra. 
Built on \Infra, the analysis in this paper opens new system optimization opportunities for provisioning hardware resources and designing specialized hardware~\cite{lottery} by judiciously quantifying the overall recommendation quality, tail-latency, and system throughput.
First, we perform an in-depth characterization of recommendation model accuracy and latency-bounded throughput performance using open-source recommendation data sets and model architectures~\cite{dlrm, criteo}.
Next, we demonstrate how various application-level, algorithm-level, and hardware-level design parameters can be configured to gracefully meet model quality, tail-latency, and throughput targets on general-purpose CPUs and GPU-based AI accelerators.
Finally, using the insights from empirical measurements on real systems, we propose \Accel---a multi-stage recommendation inference accelerator---that exploits both query-level and model-level parallelism to jointly optimize recommendation quality, tail-latency, and system throughput.

%\textcolor{blue}{Using \Accel, we show [highlight key results, key takeaways, insights here.]}


%lexity for each stage can maximize the overall quality of recommendations while minimizing latency and improving throughput.
%Furthermore, ranking more candidate items per user increases the likelihood of finding high-quality, personalized content.
%However, while increasing the number of candidate items improves quality, it exacerbates system performance.
%Optimizing the number of candidate items ranked per stage allows designers to carefully balance quality, latency, and throughput.
%Finally, each stage in multi-stage recommendation systems' ranking funnel enables unique opportunities for accelerations.

%Unfortunately, recent proposals for accelerating data center scale recommendation inference do not consider design optimizations across multi-stage recommendation systems.
%Prior work in multi-stage recommendation stages focuses on optimizing training accuracy and efficiency~\cite{recsys-twitter, youtube, mcauley}.
%On the other hand, computer systems and architecture researchers have proposed various techniques to optimize recommendation inference for individual models on general-purpose and specialized hardware~\cite{intel, bandana, gupta2020deeprecsys, recnmp, centaur, tensordimm}.
%For example, DeepRecSys~\cite{gupta2020deeprecsys} schedules queries across both CPUs and GPU-based AI-accelerators to maximize latency-bounded throughput for individual recommendation models.
%Similarly, Centaur proposes specialized hardware to reduce inference latency of recommendation models. 
%Compared this baseline, we demonstrate that exploiting the unique parallelism opportunities in multi-stage recommendation reduces latency by up to 3$\times$ and increases throughput by up to 4$\times$.

%Recent accelerator proposals focus on optimizing individual recommendation models for inference latency~\cite{centaur}.
%In addition to end-to-end models, TensorDimm and RecNMP accelerate embedding table operations---unique operators in DNN-based recommendation models that form the performance bottleneck~\cite{tensordim,recnmp}.
%Given the unique parallelism opportunities in multi-stage recommendation systems, this work highlights the benefits of tightly coupled algorithm-hardware co-designs.


%To enable system designers to explore the unique application-level, algorithm-level, and hardware-level design tradeoffs, this paper presents~\Infra, a framework to study data center scale multi-stage recommendation inference. 


%Multi-stage recommendation systems are used in a variety of production-scale recommendation engines.
%Cite Google Youtube (candidate generation) paper and Instagram article.
%The machine learning community has focused on how to train models across the pipeline to tailor the model to each subset of data seen.

%In addition to the machine learning community, the hardware community has proposed a variety of system solutions for recommendation.
%This includes system provisioning questions (DeepRecSys).
%Accelerating embedding operations with near memory and data processing.
%However, the work does not consider accuracy versus performance tradeoffs and does not consider end to end multi-stage ranking systems.

%In this paper, we propose an early design stage framework to optimize systems for multi-stage recommendation inference.
%Framework allows exploring algorithm (model size, accuracy, items) and hardware (CPU vs. GPU vs. accelerator) design space explorations.
%First run on CPUs.
%Then consider commodity AI-accelerators i.e., GPUs. 
%Then design specialized hardware.

The key intellectual contributions of this work include:

\begin{enumerate}
\item We propose a new framework, \Infra, that enables design space exploration and optimization for multi-stage recommendation inference. The framework integrates real recommendation data sets, models, and hardware to enable researchers to study trade-offs between recommendation quality, tail-latency, and system throughput.
%We highlight ... 
\item Using \Infra, we show that optimal multi-stage recommendation system parameters (e.g., number of stages, model complexity, candidate items) vary based on the quality, tail-latency, and system throughput targets.
Exploiting these design knobs, end-to-end recommendation on CPUs can be accelerated by ~\textcolor{blue}{X} while preserving the overall model quality.
%In particular, we find at lower latency it is advantages to have single stage models while at longer SLA targets, high accuracy is unlocked with multi-stage recommendation models.

\item We show that GPU-based AI accelerators can be appealing targets for multi-stage recommendation.
Given their data-parallel execution style, GPUs enable up to 2$\times$ lower tail-latency recommendation compared to CPUs. This reduction in tail-latency can enable significantly higher recommendation quality at the expense of lower system throughput.
Furthermore, in the presence of GPUs, we demonstrate the optimal number of ranking stages varies when optimizing for performance versus power efficiency.

\item Finally, we propose, \Accel, a novel recommendation accelerator that exploits the unique data-parallelism and model-parallelism opportunities across multi-stage recommendation. 
Compared to a representative baseline hardware accelerator, carefully provisioning resources to balance parallelism opportunities can help reduce tail-latency by 3$\times$ and increases system throughput by 4$\times$.

\end{enumerate}

==> text/accel.tex <==
\section{RecPipeAccel: Accelerating Recommendation Pipelines}~\label{sec:accel}
The results thus far have shown multi-stage recommendation systems pose unique challenges to efficient data center deployment.
As previously shown, these unique characteristics must be co-designed with available hardware (e.g., general purpose CPUs, GPU-based AI accelerators) for improving quality, inference tail-latency, and system-throughput.
Similarly, specialized hardware accelerators must target the distinct performance bottlenecks found across multi-stage recommendation systems.

To accelerate end-to-end multi-stage recommendation systems, in this section we design \Accel~(RecPipeAccel).
Central to \Accel~is the observation that each phase of multi-stage recommendation systems pose distinct opportunities for parallelism.
Earlier-stages exhibit high data-parallelism; later-stages exhibit high model-parallelism.
To collectively optimize the recommendation pipeline, \Accel~is composed of a heterogeneous array of execution units, or lanes.
Compared to a single monolithic hardware design, provisioning resource asymmetrically across lanes improves overall hardware utilization providing low-latency and high-system throughput for data center scale recommendation.

To study the unique co-design opportunities between multi-stage recommendation and hardware accelerators, this section first details the \Accel~design providing intuition on the design tradeoffs.
Next, we conduct a detailed operator-level performance characterization of RM$_{\textrm{small}}$, RM$_{\textrm{med}}$, and RM$_{\textrm{large}}$ across varying \Accel-lanes.
Finally, using \Infra, we study the impact of \Accel~for data center scale recommendation.


\subsection{\Accel~design.}
Figure~\ref{fig:MSRAccel}(left) illustrates the high-level architecture of \Accel---a recommendation accelerator composed of an array of heterogeneous execution units or lanes (\Accel-lanes).
To independently process entire recommendation inference queries, each \Accel-lane implements an embedding gather-unit, systolic-array based MLP accelerator, and sorting unit.
The embedding gather-unit comprises an embedding cache to store frequently accessed categorical input features.
Given the high non-unit batch-sizes, systolic-arrays are used to parallelize computations for both MLP-bottom and MLP-top layers in recommendation models.
Finally, based on the final scores for each user-item pair, the sorting unit identifies top items to forward to subsequent recommendation stage engines or the host processor.
Given fixed hardware resources, the architectural components outlined in red are asymmetrically provisioned to accelerate each phase of multi-stage recommendation systems.
For instance, each lane implements a varying embedding cache size, dense inputs SRAM, MLP-weights SRAM, and systolic array size.

Figure~\ref{fig:MSRAccel}(right) provides high-level intuition behind the acceleration strategy.
Prior art designs monolithic recommendation hardware that optimizes inference latency by accelerating embedding gather and MLP-layer computations for large models (e.g.,RM$_{\textrm{large}}$)~\cite{centaur}.
Starting with this baseline, decomposing the recommendation task into finer-grained pipelines using \Infra~reduces latency by up to 3$\times$.
Accelerating model inference alone, leaves the crucial operation of sorting user-item interactions between phases of the multi-stage recommendation pipeline.
While the baseline leverages a host processor to identify high-quality recommendations from the predicted scores, the dedicated sorting accelerator eliminates inefficient accelerator-host communications, reducing the overall latency by an additional 1.4$\times$. 
The sorting accelerator also enables the specialized hardware to process recommendation queries end-to-end (i.e., across all stages).
Processing queries end-to-end, frontend recommendation models (e.g., filtering stages) implement networks with smaller embedding tables and MLP-layers  recommendation.
Accelerating these smaller models on larger, monolithic accelerators leads to low hardware utilization.
Instead, \Accel~concurrently processes multiple queries by provisioning hardware resource across lanes dedicated to each stage in recommendation pipelines---providing signficant throughput improvements.


%While prior art accelerates large (e.g., memory intensive, compute intensive, accurate) recommendation models~\cite{}, \Accel~is composed of a set of heterogeneous processing elements (PEs) to separately optimize early-stage and late-stage recommendation models.
%Each PE comprises a embedding gather and systolic-array based MLP accelerator unit.
%To accelerate early-stage models, PEs are designing to extract high data-parallelism opportunities; on the other hand, to accelerate backend-models, PEs are designed to extract high degrees of model-parallelism.


\begin{figure}[t!]
  \centering
  \includegraphics[width=\columnwidth]{plots/systolic_array_perf.pdf}
  \vspace{-2.5em}
  \caption{Characterizing the performance and utilization of the systolic array across a range of hardware and model sizes.
  The low utilization of larger accelerators on smaller models motivates provisioning resources across multiple smaller lanes---enabling concurrent query processing.}
  \label{fig:systolic}
  \vspace{-1em}
\end{figure}

\begin{figure*}[t!]
  \centering
  \includegraphics[width=\textwidth]{plots/accel_op_breakdown.pdf}
  \vspace{-2.5em}
  \caption{Detailed operator breakdown of three \Accel~design across three recommendation models and inference batch-sizes. Generally, the time devoted to MLP operations increases with larger models and batch-sizes. 
  Larger accelerator design also suffer from a significant fraction of time devoted to input data and output results communication over PCIe---to achiever higher utilization, the larger accelerators are split into multiple smaller ones.}
  \label{fig:operator}
  \vspace{-1em}
\end{figure*}

\begin{figure*}[t!]
  \centering
  \includegraphics[width=\textwidth]{plots/accel_analysis.pdf}
  \vspace{-1em}
  \caption{(Left) At iso-quality and hardware resources, co-designing multi-stage recommendation models with the hardware enables lower latency and higher inference throughput.
  (Middle) Asymmetrically provisioning the number of \Accel~lanes for frontend and backend models unlocks lower latency and higher throughputs compared to homogeneous hardware typologies.
  (Right) In addition to achieving high system-throughput, \Accel~can trade off low inference latency for significantly improving recommendation quality.\fixme{fix colors to make consistent.}}
  \label{fig:accel_analysis}
  \vspace{-1em}
\end{figure*}


\subsection{Performance modeling and design space tradeoffs.}
To gain a deeper understanding of \Accel, in this section we conduct a detailed performance characterization of the proposed design.

The latency of processing recommendation queries is the aggregate inference time of each step in the multi-stage pipeline.
Inference latency for each stage is computed as follows:
$Latency_{stage} = MLP_{bot}+MLP_{top}+Embedding+Sort$. 
Here we detail how the latency of each component is modeled.
(Detailed architectural parameters are found in Section~\ref{sec:method}).

\textbf{Embedding table operations.}
The performance of embedding table operations is determined by the time taken to perform the irregular memory accesses and fetch embedding vectors.
We model the memory access time based on average DRAM latency and bandwidth parameters.
To reduce embedding lookup times, \Accel~implements a software managed embedding cache for frequently accessed vectors.
The memory locality pattern is based on the trace of real embedding lookups using open-source datasets and user-item filtering across recommendation stages.

Figure~\ref{fig:x} shows the average hit rate for varying embedding cache sizes.

\begin{figure*}[t!]
  \centering
  \includegraphics[width=\textwidth]{plots/summary.pdf}
  \vspace{-2em}
  \caption{Summary of RecPipe results at iso-quality targets for the Criteo Kaggle (left) and MovieLens1m (right) datasets. The optimum number of stages in the recommendation pipelines varies across system throughputs, underlying hardware platform, and dataset. \fixme{Grey out bars that go high.}}
  \label{fig:}
  \vspace{-1em}
\end{figure*}

\textbf{MLP layers.}
To model the time to process MLP layers using systolic arrays, we build the MLP units within \Accel~on top of ScaleSim~\cite{}, a cycle-accurate DNN accelerator. 
Across the range of model architectures and batch-sizes, we find weight-stationary systolic-arrays to outperform both input-stationary and output-stationary styles~\cite{}.
In addition to the compute time of processing MLP layers using systolic arrays, we consider the input and weight loading times based on the average DRAM bandwidth and latency.
For the purposes of this work, all \Accel~designs implement 64$\times$64 MAC units. 
Consequently, in a monolithic accelerator design, the single lane comprises all 4096 MAC units; when the numbers of lanes are doubled to process two queries in parallel, each lane comprises 2048 MAC units.

Figure~\ref{fig:systolic} illustrates the performance (top) and hardware utilization (bottom) of the systolic array units for various \Accel-lane sizes.
As expected, increasing the number of MAC units within a lane reduces the cycles to process MLP layers within RM$_{\textrm{large}}$, RM$_{\textrm{med}}$, and RM$_{\textrm{small}}$.
However, with the improved performance, hardware utilization degrades.
Given the largest \Accel-lane size, the MAC utilization of the systolic array for RM$_{\textrm{large}}$, RM$_{\textrm{med}}$, and RM$_{\textrm{small}}$ is 40\%, 15\%, and 5\% respectively.
Given multi-stage recommendation uses a collection of small and large models, the low utilization limits the achievable system-level performance. 
Instead of the monolithic design, \Accel~provisions resources across heterogeneous lanes to maximize utilization leading to higher inference throughput.

\textbf{Sorting user-item interactions.}
Finally, to model the time to sort user-item interactions. 
User-item interactions are sorted based on the output probability score from the final layer in the top MLP stack of recommender models. 
To reduce the hardware complexity of sorting user-item scores, \Accel's sorting unit maintains a list of top-$k$ interactions in a local SRAM buffer as scores are sequentially generated by \Accel's systolic array.
Upon processing all user-item interactions, the sorting unit forwards the top-$k$ list to subsequent accelerator engines for finer grained ranking or the host.
The performance of this single-pass sort is set by the number of top-$k$ interactions to forward and the memory bandwidth of the SRAM buffer.
In practice, the accelerated sorting unit comprises hundreds of cycles---negligible compared to the overall inference time. 

\textbf{PCIe data communication.} In addition to the individual operators it is important to consider data communication time for transferring recommendation inputs from the host processor and \Accel.
To account for the data communication we measure PCIe data communication time between the Intel Cascade Lake and NVIDIA T4 GPU.
Based on the working set size, the same data communication latencies are applied for \Accel.


Figure~\ref{fig:operator} illustrates the overall operator breakdown across various inference batch-sizes (i.e., 256, 1024, 4096), model architectures (i.e., RM$_{\textrm{small}}$, RM$_{\textrm{med}}$, and RM$_{\textrm{large}}$) and three \Accel-lane sizes.
For thoroughness, the performance analysis includes the range of \Accel-lane sizes considered in this work: small, medium, and large which implement lanes with one-sixteenth, one-fourth, and the all hardware resources.
Note, in the largest accelerator topology, over 70\% and 50\% of cycles are devoted to PCIe data communication for query input and outputs for RM$_{\textrm{small}}$ and RM$_{\textrm{med}}$, respectively.
This high fraction of data communication cycles limits the performance advantage from larger accelerator designs for earlier stage recommendation models.
To balance inference latency and system throughput, \Accel~provisions multiple smaller lanes for frontend and backend stages.




\subsection{Data center scale recommendation optimization}
Based on the performance characterization, \Infra~is instrumented with the proposed multi-stage accelerator, \Accel, to consider its impact on data center scale recommendation. 

\textbf{Improving system efficiency with \Accel.}
Figure~\ref{fig:accel_analysis}(left) illustrates the tradeoff between inference throughput and latency for accelerating one-stage, two-stage, and three-stage recommendation pipelines with \Accel.  
Given a fixed hardware resource budget and recommendation quality target, we consider a variety of \Accel-lane provisioning decisions for all stages.
The baseline monolithic recommendation model and accelerator achieves a latency of 4.1$ms$ and system-throughput of 500 QPS.
In comparison, the decomposed finer-grained pipelines achieves a latency of 2.1$ms$ and system-throughput of up to 2500 QPS---a 2$\times$ and 5$\times$ improvement, respectively.
The latency reduction and system-throughput increase owe to the combination of more efficient recommendation model architecture and higher hardware utilization from asymmetrically provisioning resources across \Accel-lanes.

\textbf{Asymmetric provisioning for accelerator resources.}
Figure~\ref{fig:accel_analysis}(middle) illustrates the benefit of asymmetrically provisioning hardware resources across \Accel-lanes processing each stage.
For a two-stage recommendation system the front end is fixed with eight lanes (i.e., \Accel$_{8,8}$) while the backend implements two (i.e., \Accel$_{8,2}$) and sixteen lanes (i.e., \Accel$_{8,16}$).
All experiments assume iso-hardware resources and iso-recommendation quality.

Compared with the homogeneous accelerator provisioning (i.e., \Accel$_{8,8}$), the aggregating the backend into fewer, larger lanes \Accel$_{8,2}$ reduces the inference latency at low system-throughput by up to 1.5$\times$.
Similarly, splitting the backend into more, smaller lanes \Accel$_{8,2}$ reduces the inference latency at high system-throughput by up to 1.4$\times$.
Given application-level inference latency and system targets, asymmetrically provisioning \Accel~resources across lanes can widen the design space of recommendation services.
Alternatively, building on prior art, \Accel~resources could be dynamically reconfigured to meet varying targets given workload demands~\cite{planaria}.

\textbf{Improving recommendation quality with \Accel.} 
In addition to improving system efficiency, \Accel~can improve overall recommendation quality.
Figure~\ref{fig:accel_analysis}(right) shows the tradeoff between inference latency and recommendation quality for a single-stage and multi-stage \Accel~design at iso-throughput (i.e. QPS of 500) and iso-hardware resources.
While the previous analysis in our work considers a maximum of 4096 items to rank per query, here we increase the items to rank from 4096 to 28672 given the low inference latency of \Accel.
Compared to the single-stage design which achieves a recommendation quality of 98.6, the two-stage design achieves a quality of 99.7--near optimal.
Thus, co-designing multi-stage models and hardware accelerators can enable both higher system efficiency and higher quality recommendation services.


==> text/introduction.tex <==
\section{Introduction}

% DNN recommendation constitutes >80% AI inference cycles at Facebook.
% Model quality is the key
% Naive approaches to design systems for "high-quality" models requires massive resources, in the dimensions of compute, memory, energy, ...
% Alternatively, we can adopt pruning~\cite{}, NMPs~\cite{}, ....
Deep neural network (DNN) based recommendation systems constitute an overwhelming majority of all AI cycles in Facebook's data centers~\cite{hazelwood2018applied, gupta2020architectural, acun2020understanding}. 
Similar infrastructure demands are found throughout the industry (e.g., Google and Alibaba) to personalize user experience in a wide range of services, including search, e-commerce, movie and video streaming, and social media~\cite{tpu, dinzhou2018deep, dienzhou2019deep, mtwnd, ncf}.
To improve the quality and personalization of content, the size of production recommendation models has grown by over 10$\times$ between 2017 and 2020~\cite{lui2020understanding} into the terabyte scale~\cite{yiSysml18,baidu_aibox,baidu_dist_inf}.
%The growing model complexity exacerbates system demands for serving recommendation at the data center scale in terms of compute, memory and storage, and energy. 

In response to the dramatic increase in infrastructure demands from the ever-increasing model complexity, 
%Optimizing DNN-based recommendation inference, 
researchers have proposed system- and architecture-level solutions customized for DNN-based recommendation, including inference schedulers~\cite{gupta2020deeprecsys}, near memory processing hardware~\cite{ke2020recnmp,kwon2019tensordimm}, and specialized accelerators~\cite{centaur}.
Assuming fixed models and workload characteristics, previously proposed hardware solutions solely improve performance.
%In contrast, as shown in Figure~\ref{fig:overview}, this work co-designs recommendation models and hardware solutions creating opportunities to improve both recommendation quality and performance.
%In contrast, as shown in Figure~\ref{fig:overview}, our work co-designs recommendation model parameters and hardware solutions to holistically improve both quality and performance.
%In contrast, as shown in Figure~\ref{fig:overview}(a), 
In contrast, this paper presents 
{\it \Name}, a system to co-design recommendation models and hardware solutions to improve both quality and performance (Figure~\ref{fig:overview}(a)) on commodity platforms (e.g., CPU, GPU) and custom accelerators.
%The proposed co-design techniques enable \Name~to optimize recommendation inference across both commodity hardware (e.g., CPU and GPU) and custom accelerators. 

%Central to personalized recommendation is the ability to accurately rank content based on user preferences and previous interactions.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.95\columnwidth]{figures/Overview.pdf}
  \vspace{-1.0em}
  \caption{ Compared to recent work from machine learning and computer architecture researchers, this work collectively improves recommendation quality, tail-latency, and throughput (a) by co-designing models and hardware solutions across multi-stage recommendation pipelines (b). 
  Transforming monolithic models into multiple stages reduces overall compute demand and embedding memory accesses by 7.5$\times$ and 4.0$\times$, respectively (c).}
  \label{fig:overview}
  \vspace{-1em}     
\end{figure}

% or we can break this huge, monolithic model into stages of smaller models?
% What are multi-stage recommendation models?
Achieving both high quality and performance is challenging using monolithic recommendation models.
Such models rely on large, complex DNNs to rank a large number of candidate items (i.e., working set size), exacerbating inference latencies and hardware demands.
However, only a small portion of candidate items are relevant to individual users---ranking all items with complex recommendation models is wasteful.
%However, not all items are equally relevant to users.
%\textcolor{blue}{In fact, only a small portion of candidate items (1-10\% of commonly-used recommendation data sets) is considered relevant. 
Decomposing monolithic ranking models into multiple DNN stages is a promising solution to simultaneously improve quality and performance~\cite{instagramMsr, mtwnd, kang2019candidate}.
%One promising solution to efficiently serve recommendation models while improving quality, is to decompose monolithic recommendation models into finer-grained multi-stage pipelines~\cite{instagramMsr, mtwnd, kang2019candidate}.
By splitting the monolithic model into two, a frontend model coarsely \textit{filters} relevant items per user while a more accurate backend model \textit{ranks} at a finer-granularity.
One can further segment the pipeline into additional stages, creating a ranking funnel (Figure~\ref{fig:overview} (b)). 
In multi-stage pipelines, complex models are only used to rank items that require accurate differentiation.
%\textcolor{blue}{The multi-stage pipeline builds on the insight that complex models are only needed when items require fine-grained differentiation.}
%From the system's perspective, compared to single-stage recommendation, this decomposition improves latency-bounded performance and efficiency for not only individual stages but also the overall multi-stage pipeline.
From the system's perspective, decomposing monolithic recommendation engines into pipelines improves overall efficiency.
%pipelines enable more targeted optimizations for individual stages and improve latency-bounded performance and efficiency for the overall pipeline.
%Compared to monolithic designs, multi-stage pipelines 
%From the system's perspective, latency-bounded performance and efficiency can be significantly improved when monolithic recommendation models are decomposed into multi-stage pipelines.
Figure~\ref{fig:overview}(c) shows that, at iso-quality, compared to single-stage, multi-stage recommendation can reduce memory and compute demands by 4.0$\times$ and 7.5$\times$, respectively.


%Alternatively, to reduce system demands while maintaining high model quality, monolithic recommendation systems can be decomposed into finer-grained multi-stage recommendation pipelines.
%Monolithic recommendation systems achieve high quality by ranking a large number of candidate items using large, complex DNN-based recommendation models.
%The combination of a large number of items to rank (i.e., working set size) and the ever-increasing model complexity degrades inference latency as well as achievable system throughput.
%makes meeting strict SLA targets challenging and lowers achievable system throughput.
% ^^^ Seems redundant with sentence 1 of this P
%However, not all items are equally relevant to users.
%As shown in Figure~\ref{fig:overview}, multi-stage recommendation systems implement a ranking funnel to evaluate relevance of candidate items.
%Earlier stages implement lightweight models to coarsely filter out relevant items while later stages implement more accurate models for fine-grained ranking. 
%At iso-quality compared to monolithic models, from the system's perspective latency-bounded performance and efficiency can be significantly improved when recommendation systems are decomposed into fine-grained multi-stage execution pipeline.
%Figure~\ref{fig:overview}(bottom) shows that, with the same model quality (iso-quality), decomposing monolithic models into multi-stage execution can reduce memory and compute resource demands by 
%5.3$\times$ and 5.9$\times$, respectively.





% Why is it hard? What are the challenges designing these multi-stage recommendation models?
% Unique compute requirements across multi-stage recommendation systems
%One of the challenges in designing multi-stage recommendation is the lack of design tools to jointly evaluate inference run-time performance and overall recommendation quality.
%Recommendation quality is determined by the model accuracy and number of items ranked (i.e., input working set size) across all stages in multi-stage recommendation.
%In terms of recommendation quality, it is crucial to balance both the model complexity and number of items to rank per stage (i.e., input working set size).
%Across the stages, varying model complexities and input working set sizes expose distinct opportunities for performance optimization. 
%Frontend stages pair light-weight models (e.g., low compute and memory demands) with large input sizes, providing higher degree of data-parallelism.
%Backend stages pair heavy-weight models (e.g., billions of FLOPs, many GBs of storage) with low input sizes; such ranking models expose model-parallelism opportunities instead.
%To date, domain-specific system and architecture solutions accelerate recommendation models in isolation~\cite{gupta2020deeprecsys, ke2020recnmp, kwon2019tensordimm, centaur}---leading to inefficient system designs for end-to-end multi-stage pipelines. % significant performance improvement potential compared to co-designing end-to-end pipelines.
%New approaches to jointly design models and hardware solutions for all stages in a recommendation pipeline are needed.
%intrinsically different system solutions are needed for each stage in multi-stage recommendation.

% Marks attempt at Paragraph 3 ...
A primary challenge in designing systems for multi-stage recommendation is jointly optimizing inference run-time performance and recommendation quality.
%evaluating inference run-time performance and quality 
%A primary challenge in designing multi-stage recommendation is jointly evaluating inference run-time performance and recommendation quality.
Recommendation quality is dependent on both model accuracy and the number of items ranked.
%Recommendation quality is dependant on both the quality of available inputs -- not all candidate items can be feasibly ranked --, and on the accuracy of the model processing those varied inputs.
Multi-stage recommendation exploits this property of quality as models are split into pipelines to efficiently process a large set of inputs and service high quality recommendations.
This exposes new opportunities to co-design models and hardware as the stages vary in model complexities and input working set sizes. 
%exposes distinct opportunities for performance optimization. 
Frontend stages pair light-weight models (e.g., low compute and memory demands) with large input sizes, providing higher degree of data-parallelism.
Backend stages pair heavy-weight models (e.g., billions of FLOPs, many GBs of storage) with low input sizes, exposing model-parallelism opportunities instead.
To date, domain-specific architecture solutions accelerate recommendation models in isolation~\cite{gupta2020deeprecsys, ke2020recnmp, kwon2019tensordimm, centaur,wilkening2021recssd}---leading to inefficient system designs for end-to-end multi-stage pipelines.
New approaches to jointly design models and hardware solutions for all stages in the pipeline are needed.

%Optimizations based on these distinct challenges, compared to previous state-of-the-art solutions, lead to tail-latency and system-throughput improvement by 3$\times$ and 4$\times$, respectively.

% Yeahh want to clean up opportunities vs challenges. You might want to start with something like -- there exist different optimization points for different stages -- previous work on monolithic optimizations have handled these design points independently -- we need a system that can DO both and BALANCE both 
%First, each phase of multi-stage recommendation system poses distinct performance bottlenecks.
% Might be clearer to state multi-stage specific optimizations provide ...blah... over state-of-the-art optimized monolithic systems

%To-date, DSA accelerators have been designed for monolithic DNN-based models, individually. Instead, this work explores algorithm-architecture co-design opportunities for DNN-based recommendation models by decomposing monolithic models into multi-model systems. 



% In addition, an opportunity unique for co-design is the aspect of "training" that enables this design trade-off with "model quality" 
% So [introduce what this paper does]
%Furthermore, to maximize overall recommendation quality under strict performance and resource constraints, designers must balance the accuracy and performance of individual models.
%Compared to CNNs and RNNs, 
%Multi-stage recommendation systems allow rigorous and quantitative trade-offs between model accuracy versus performance using two key design parameters: model complexity and number of candidate items.

%Increasing model complexity and increasing the number of candidate items both improve ranking quality while degrading run-time performance.
%Given these distinct parameters, our analysis demonstrates that under resource constraints, it is often advantageous to deploy less sophisticated, accurate models with larger candidate items to achieve comparable recommendation quality but with much higher throughput performance.

%^^^ Yeah, this is redundant with your initial presentation of multi-stage funnels (paragraph 2), just more detailed in the parameters you use to alter being 'light-weight' or 'more accurate/fine-grained'. I would rather have something more like this IMO than the caching analogy.




%Given the importance of DNN-based recommendation models, domain-specific architecture (DSA) solutions are emerging. 
%First, compared to convolutional and recurrent neural networks, DNN-based recommendation models comprise embedding table operations that exhibit highly irregular memory access patterns and large storage capacities~\cite{gupta2020architectural}.
%Recent work proposed specialized near-memory processing hardware to accelerate embedding operations central to recommendation~\cite{tensordimm, recnmp}.
%In addition to accelerating individual operators, Centaur~\cite{centaur}, a hybrid sparse-dense accelerator, was demonstrated to reduce recommendation inference latency. 
%However, recommendation systems must meet both strict tail-latency targets set by service-level agreements (SLAs) and high system throughput to enable applications that serve billions of users worldwide.
%Taking a step further to optimize inference latency-bounded throughput, specialized recommendation query schedulers were proposed to partition work across general purpose CPUs and specialized AI-hardware~\cite{gupta2020deeprecsys}. 

%\textcolor{blue}{[Talk about the related works here, follow by what the remaining gaps are and what's addressed by this work.]}

%accelerated hardware accelerators for 

%llion of parameters that pose high compute requirements, irregular memory access patterns, and storage capacities.



%\textcolor{blue}{Condense into the previous P.} While modern deep-learning solutions improve user experiences through higher quality recommendation, they exacerbate system requirements.
%First, DNN-based recommendation models comprise billions of parameters that pose high compute requirements, irregular memory access patterns, and storage capacities.
%For each input query DNN-based recommendation models rank potentially thousands of items to identify the best, most personalized content.
%The combination of large models and query sizes results in long inference latencies that make meeting strict tail-latency thresholds set by application-level service-level agreements (SLAs) challenging.
%In fact, SLA targets for recommendation systems vary from tens to hundreds of milliseconds posing a diverse range of design challenges~\cite{gupta2020deeprecsys}.
%In addition to meeting strict tail-latency targets, recommendation systems must operate at high throughput owing to applications serving potentially billions of users worldwide.
% Not a fan of this here...
%Thus, efficient deployment of recommendation systems requires judiciously balancing the benefits of more sophisticated recommendation systems (e.g., quality) with the challenges they pose (e.g., latency, throughput).
%recommendation quality of more sophisticated models and the challen resulting latency and system throughput 
%Thus, efficiently deploying recommendation systems requires carefully balancing recommendation quality, latency, and throughput.

%Although the aforementioned architectural innovations optimize individual recommendation models, data center scale systems typically comprise many models that collaboratively rank content.

%By doing so, we optimize recommendation quality, inference tail-latency, and system throughput 


%Inputs to recommendation systems are a large number of items (in the order of thousands) that are each ranked with complex DNN-based models. Combined with the stringent model quality requirement, recommendation models incur 
%Unfortunately, meeting strict SLA targets while ranking a large number of candidate items with complex DNN-based models incurs 
%heavy compute and infrastructure demands.
%To reduce the ever-increasing resource requirement, multi-stage systems use a ranking funnel to evaluate candidate items, as shown in Figure~\ref{fig:overview}(b).

%Note that such multi-stage designs are used in YouTube's video recommendation system, Instagram social media platform, and \cite{}.
%Intuitively, earlier stages filter candidate items using light-weight models while later stages are heavier-weight in order to perform fine-grained ranking to identify the most relevant candidate items.
%Compared with models in later stages, light-weight models comprise orders of magnitude lower FLOPs, memory lookups, and memory capacity demands.
%Algorithmically, filtering candidate items using light-weight models can significantly reduce the overall compute and memory demands of recommendation systems. 

%One approach to balancing recommendation quality, latency, and throughput is to use multi-stage recommendation systems~\cite{multitask, instagram, gupta2020architectural}.
%Compared to typical single-stage recommendation systems, multi-stage systems reduce the computational complexity of ranking large sets of candidate items.
%Intuitively,  and reduce overall computational complexity.



%Multi-stage recommendation provide a unique opportunity for systems designers to trade off individual model accuracy and run-time performance to maximize end to end system quality, latency, and throughput.
%Co-designing algorithm and hardware solutions across the stages widens the design space of system solutions as compared to optimizing each stage individually.
%Multi-stage recommendation systems provide unique system design opportunities to balance recommendation quality, latency, and throughput.

%As depicted in Figure~\ref{fig:overview}(a), \textcolor{blue}{this work is one of the few first ones that approaches system design and optimization by co-designing model architectures and hardware.} 
We propose \Infra, a system to co-design models and hardware solutions for multi-stage recommendation across commodity platforms and customized accelerators.
%A core component of RecPipe is RecPipeInfra (\Infra), a framework to co-design both models and hardware solutions for multi-stage recommendation.
Central to \Infra~is a multi-step design process to rigorously quantify and simultaneously optimize recommendation quality, system throughput, and inference performance to meet strict tail-latency targets set by service-level agreements (SLAs). 
The first step is determining the overall recommendation quality and resource demands by balancing model complexity, model accuracy, and number of items to rank in each stage of the pipeline.
Next, \Infra~implements a static, post-training inference scheduler that maps each recommendation stage across commodity, heterogeneous hardware resources (e.g., CPU, GPU) to maximize performance.
%Given that data centers now implement heterogeneous hardware %systems~\cite{hazelwood2018applied}, \Infra~can optimize across commodity CPU and GPU systems to maximize performance.
Finally, given the importance of data-center scale personalized recommendation, there is growing interest from academia and industry to build specialized hardware for neural recommendation~\cite{centaur, ke2020recnmp, wilkening2021recssd,sambanova,jiang2021microrec}.
Thus, given the distinct opportunities exposed by \Infra, we design {\it RecPipeAccel} (\Accel), a specialized accelerator that is designed specifically for multi-stage recommendation.
%parallelization opportunities in multi-stage recommendation.

%Next, as data centers implement heterogeneous hardware systems~\cite{kim2018hpca}, \Infra~maps each recommendation stage across CPUs and GPUs to maximize performance. 
%Given the importance of personalized recommendation, there is growing interest from academia and industry to build specialized hardware for neural recommendation.
%In the final step, \Infra~ enables the design of specialized accelerators that exploit the distinct parallelization opportunities across multi-stage recommendation.

%The analysis in this paper opens new opportunities for provisioning hardware resources and designing specialized hardware to collectively improve recommendation quality, inference tail-latency, and system throughput.

%First, we perform an in-depth characterization of recommendation model accuracy and latency-bounded throughput performance using open-source recommendation data sets and model architectures~\cite{dlrm, criteo}.

%Its highly extensible implementation allows researchers to consider the impact of varying model architecture across a variety of hardware platforms including general purpose CPUs, GPU-based AI accelerators, and specialized hardware.

%Next, we demonstrate how various application-level, algorithm-level, and hardware-level design parameters can be configured to gracefully meet model quality, tail-latency, and throughput targets on general-purpose CPUs and GPU-based AI accelerators.
%Finally, using the insights from empirical measurements on real systems, we propose \Accel---a multi-stage recommendation inference accelerator---that exploits both query-level and model-level parallelism to jointly optimize recommendation quality, tail-latency, and system throughput.

%\textcolor{blue}{Using \Accel, we show [highlight key results, key takeaways, insights here.]}


%lexity for each stage can maximize the overall quality of recommendations while minimizing latency and improving throughput.
%Furthermore, ranking more candidate items per user increases the likelihood of finding high-quality, personalized content.
%However, while increasing the number of candidate items improves quality, it exacerbates system performance.
%Optimizing the number of candidate items ranked per stage allows designers to carefully balance quality, latency, and throughput.
%Finally, each stage in multi-stage recommendation systems' ranking funnel enables unique opportunities for accelerations.

%Unfortunately, recent proposals for accelerating data center scale recommendation inference do not consider design optimizations across multi-stage recommendation systems.
%Prior work in multi-stage recommendation stages focuses on optimizing training accuracy and efficiency~\cite{recsys-twitter, youtube, mcauley}.
%On the other hand, computer systems and architecture researchers have proposed various techniques to optimize recommendation inference for individual models on general-purpose and specialized hardware~\cite{intel, bandana, gupta2020deeprecsys, recnmp, centaur, tensordimm}.
%For example, DeepRecSys~\cite{gupta2020deeprecsys} schedules queries across both CPUs and GPU-based AI-accelerators to maximize latency-bounded throughput for individual recommendation models.
%Similarly, Centaur proposes specialized hardware to reduce inference latency of recommendation models. 
%Compared this baseline, we demonstrate that exploiting the unique parallelism opportunities in multi-stage recommendation reduces latency by up to 3$\times$ and increases throughput by up to 4$\times$.

%Recent accelerator proposals focus on optimizing individual recommendation models for inference latency~\cite{centaur}.
%In addition to end-to-end models, TensorDimm and RecNMP accelerate embedding table operations---unique operators in DNN-based recommendation models that form the performance bottleneck~\cite{tensordim,recnmp}.
%Given the unique parallelism opportunities in multi-stage recommendation systems, this work highlights the benefits of tightly coupled algorithm-hardware co-designs.


%To enable system designers to explore the unique application-level, algorithm-level, and hardware-level design tradeoffs, this paper presents~\Infra, a framework to study data center scale multi-stage recommendation inference. 


%Multi-stage recommendation systems are used in a variety of production-scale recommendation engines.
%Cite Google Youtube (candidate generation) paper and Instagram article.
%The machine learning community has focused on how to train models across the pipeline to tailor the model to each subset of data seen.

%In addition to the machine learning community, the hardware community has proposed a variety of system solutions for recommendation.
%This includes system provisioning questions (DeepRecSys).
%Accelerating embedding operations with near memory and data processing.
%However, the work does not consider accuracy versus performance tradeoffs and does not consider end to end multi-stage ranking systems.

%In this paper, we propose an early design stage framework to optimize systems for multi-stage recommendation inference.
%Framework allows exploring algorithm (model size, accuracy, items) and hardware (CPU vs. GPU vs. accelerator) design space explorations.
%First run on CPUs.
%Then consider commodity AI-accelerators i.e., GPUs. 
%Then design specialized hardware.

The intellectual contributions of this work include:
\begin{enumerate}[leftmargin=*]
\item We propose a new system, \Infra, that enables design space exploration and optimization for multi-stage recommendation inference. 
The framework integrates real-world recommendation data sets (e.g., MovieLens 1M and 20M~\cite{movielens1m}, Criteo Kaggle~\cite{criteo}), models (e.g., neural matrix factorization~\cite{he2017neural}, Facebook's Deep Learning Recommendation Model (DLRM)~\cite{naumov2019deep}), and hardware (e.g., Cascade Lake CPU server, T4 inference GPU, simulated accelerators) to enable researchers to study trade-offs among quality, tail-latency, and throughput.
%We highlight ... 

\item Using \Infra, we show the optimal multi-stage recommendation configuration---number of stages, model complexity, items to rank---depends on the application level targets (i.e., quality, tail-latency, throughput) and underlying hardware.
At iso-quality and iso-throughput, efficiently scheduling multi-stage recommendation on commodity platforms reduces tail-latency by 1.6$\times$ and 2$\times$ on CPUs and heterogeneous CPU-GPU hardware, respectively. 

%Using \Infra, we show the best design point for multi-stage recommendation---number of stages, model complexity, items to rank---depends on the quality, tail-latency, and throughput targets.
%In fact, decreasing model complexity to rank more items often improves performance at comparable quality.
%On CPUs, such algorithmic optimizations reduce tail-latency by 1.6$\times$ at iso-quality and iso-throughput.
%In particular, we find at lower latency it is advantages to have single stage models while at longer SLA targets, high accuracy is unlocked with multi-stage recommendation models.

%\item In addition to the multi-stage parameters, we demonstrate the optimal mapping of stages to commodity hardware depends on the SLA. %application-level target.
%Compared to CPUs, GPUs reduce tail-latency by 2$\times$ at the expense of lower throughput.
%While CPUs provide higher throughput, the reduced tail-latency can lead to higher quality or energy efficiency.

%\fixme{With GPUs} the \fixme{optimum} design of multi-stage recommendation pipeline varies compared to CPU-only execution.
%Given their data-parallel execution style, 
%This reduction in tail-latency can enable significantly higher recommendation quality or energy efficiency at the expense of lower system throughput.

\item Using \Infra, we design \Accel, a novel recommendation accelerator that exploits distinct data-parallelism and model-parallelism opportunities across stages. To further improve performance, \Accel\ breaks queries into sub-batches to pipeline stages, and eliminates overheads from host-accelerator communication across stages.
Compared to a state-of-the-art baseline accelerator~\cite{centaur}, \Accel's optimizations reduces tail-latency by 3$\times$ and increases throughput by 4$\times$ at iso-quality.

\end{enumerate}

==> text/msr.tex <==
\section{The RecPipeInfra Framework}~\label{sec:flow}

To explore unique co-design optimization opportunities enabled by multi-stage recommendation systems, in this section we propose \Infra~(\Name Infra).
\Infra~enables co-optimizing recommendation quality, inference latency, and overall system throughput, by co-designing algorithms and hardware systems for multi-stage recommendation inference.
Central to \Name~is the observation that each stage provides distinct parallelism opportunities.
For example, while earlier, filtering stages exhibit high data-parallelism, later ranking stages exhibit high model-paralellism.
Given these distinct parallelism opportunities and application-level targets, we find the optimal mapping of models to underlying hardware platforms (e.g., general purpose CPUs and GPU-like AI accelerators) varies.
Motivated by these findings, we design \Accel~(\Name Accel) a novel hardware accelerator composed of heterogeneous inference engines to exploit varying degrees of data-parallelism and model-parallelism in multi-stage recommendation.

Figure~\ref{fig:MSR} illustrates the overall multi-stage recommendation infrastructure.
Inputs to \Infra~are a set of un-ordered items to be ranked based on users' personal preferences.
Each stage implements a DNN-based recommendation model to score user-item interactions.
To balance system resources and meet application-level optimization targets, earlier stages filter a large set of candidate items using lightweight models;
on the other hand, later stages use more sophisticated ranking models to perform fine-grained ranking. 
To gain a deeper understanding of the framework, in this section, we first review \Infra's application-level optimization targets.
Next, given the optimization targets, we describe the key unique system design opportunities explored in this work.
Finally, we describe the process of using \Infra~to optimize recommendation systems.


\subsection{\Infra~Optimization Objectives}
To study data center scale recommendation systems, \Infra~enables system designers to quantify three application-level optimization targets, as shown in Figure~\ref{fig:MSR}(top): 

%Deployed at the cloud-scale, personalized recommendation systems are designed to maximize the quality of user-item interactions while, at the same time, meeting strict tail-latency targets set by service level agreements (SLAs).
%As applications built upon personalized recommendations serve potentially billions of users worldwide, recommendation systems must also provide high system-throughput in terms of inference queries processed per second (QPS)~\cite{gupta2020deeprecsys}.
%Thus, designers must carefully balance overall model quality, inference tail-latency, and system throughput.


\begin{itemize}[leftmargin=*]
\item Recommendation quality: Recommendation systems must serve high-quality items based on users' personal preferences. 
Distinct from the accuracy of individual models, recommendation systems can be evaluated on the overall quality of final recommendations.
To quantify recommendation quality we use NDCG~\cite{} (see Section~\ref{sec:background} for details).

%Using NDCG, recommendation quality is set by both model accuracy and the input working set size (i.e., total number of items ranked)---allowing rigorous and quantitative tradeoffs between model accuracy and performance.

%Deployed at the cloud-scale, personalized recommendation systems are designed to maximize the quality of user-item interactions while, at the same time, meeting strict tail-latency targets set by service level agreements (SLAs).
%As applications built upon personalized recommendations serve potentially billions of users worldwide, recommendation systems must also provide high system-throughput in terms of inference queries processed per second (QPS)~\cite{gupta2020deeprecsys}.
%Thus, designers must carefully balance overall model quality, inference tail-latency, and system throughput.

\item Inference tail-latency: Deployed at the cloud-scale, personalized recommendation systems are designed to serve content under strict tail-latency targets set by service level agreements (SLAs)~\cite{gupta2020deeprecsys}.
This work ensures the overall multi-stage recommendation inferences meet \textit{p99} tail-latency requirements.

\item System throughput: Within the strict tail-latency targets, recommendation systems must maximize system throughput in order to serve potentially billions of users worldwide.
In this work we measure system throughput based on the number of queries processed per second (QPS) following a Poisson arrival rate for queries entering the first stage in \Infra.
\end{itemize}

\subsection{\Infra~Design and Optimization Space}
To co-optimize across the application-level targets (i.e., recommendation quality, inference tail-latency, system throughput), we explore a collection of algorithm-level (Figure~\ref{fig:MSR} middle) and hardware-level design optimizations (Figure~\ref{fig:MSR} bottom).
In particular we consider three design optimizations: 

\textbf{Balancing model complexity and items to rank per stage.}
Central to this work is the observation that recommendation quality is determined by two factors: model complexity and the number of items to rank.
Increasing the complexity of DNN-based recommendation models allows higher fidelity item-scoring; more accurately identifying high-quality, personalized user-item pairs improves NDCG.
On the other hand, increasing the number of ranked items improves the likelihood of pairing high-quality, personalized items for individual users, leading to higher NDCG. 
At the algorithm-level, we balance the complexity of models and number of items to rank for each phase of the multi-stage ranking system.
Note, the model complexity is set by neural network architecture (e.g., embedding capacity, depth/width of MLP layers).
Similarly, number of items to rank per stage determines the input working set size of each stage. 
Balancing both model complexity and input working set size can unlock new opportunities to balance overall recommendation quality, inference latency, and system throughput. 
For instance, on general purpose CPUs, optimizing these algorithmic parameters alone reduces inference tail-latency by up to \fixme{2$\times$} at iso-quality and iso-throughput (see Section~\ref{sec:cpu} for details).

\textbf{Mapping recommendation stages to CPU and GPUs.} 
In addition to the algorithmic workload scaling described above, this work explores the impact of mapping multi-stage recommendation systems onto heterogeneous hardware resources like general purpose CPUs and GPU-like AI accelerators.
Recall, each phase of multi-stage recommendation poses unique system challenges---earlier stages have high input working set sizes while later stages have high capacity and compute intensive models.
To co-optimize recommendation quality, inference tail-latency, and system throughput, the distinct workload characteristics must be matched with available hardware resources.
For instance, server-class, many-core CPUs can process multiple queries in parallel, GPUs accelerate individual queries given their high data-parallel architecture.
In fact, based on the application-level targets, we find the optimal algorithmic structure (i.e., number of stages, model architecture) and hardware platform varies.
In fact, we find the optimal hardware platform varies based on the application-level targets.
Mapping these unique architectural characteristics to the varying workload demands significantly improves overall system efficiency.
For instance, compared with CPU-only multi-stage recommendation, we find GPUs reduce tail-latency by up to 2.5$\times$ at low-throughput and iso-quality (see Section~\ref{sec:gpu} for details).

\textbf{Designing specialized hardware to exploit distinct parallelism opportunities.} 
Given the tradeoffs intuition gained from mapping multi-stage recommendation systems across CPUs and GPUs, we design specialized accelerators to explicitly exploit the distinct data-parallelism and model-parallelism opportunities.
The proposed accelerator, \Accel, implements an array of processing element (PE) that each comprise an embedding gather unit and systolic array to process recommendation queries.
PE's within \Accel~are provisioned with heterogeneous resources including DRAM bandwidth, systolic array size (compute intensity), and SRAM capacity.
The heterogeneous design enables \Accel~to accelerate both data-parallel and model-parallel recommendation workloads while maintaining high utilization, limiting wasted resources.
Compared to prior recommendation accelerator designs~\cite{centaur}, \Accel~reduces inference tail-latency by up to 3$\times$ or increases system throughput by up to 4$\times$ with iso-quality (see Section~\ref{sec:accel} for details).




\subsection{\Infra~Analysis Flow}


Given the varying input working-set size and model characteristics of each stage, it is important to co-design the underlying hardware systems with the workload demands. 
Unfortunately, industry-scale DNN-based recommendation models are rapidly evolving in terms of memory capacity~\cite{fb}, compute intensity~\cite{}, and modeling techniques~\cite{zhou2018deep, zhou2019deep}.
To anticipate hardware needs~\cite{hwlottery}, \Infra~enables early design space exploration to consider the impact of future recommendation models on the underlying hardware.
To study this algorithm-hardware co-design, we first conduct a training design space exploration.
The hyper-parameter sweep generates a range of Pareto-optimal recommendation networks in terms of accuracy and efficiency (see Section V).
To highest accuracy model is used to set an aggressive recommendation quality (NDCG) baseline. 
Using this baseline we study the impact of the aforementioned design optimizations: balancing model complexity with items to rank per stage, mapping recommendation stages to heterogeneous hardware resources, and designing specialized hardware to exploit distinct parallelism opportunities across multi-stage recommendation.
To gain intuition on the system design tradeoffs, we study cross-sections of iso-quality, iso-latency, and iso-throughput. 

%Thus, the optimum hardware system will also vary across recommendation systems.
%To study the hardware design tradeoffs, this work considers recommendation models with varying memory capacity and compute intensities.
%Across the models we consider two hardware optimizations: workload mapping and accelerator design.
%First we optimize workload mapping and resource provisioning decisions on whether recommendation models should run on general purpose CPUs or GPU-like AI-accelerators.
%Next, we consider how multi-stage recommendation systems influence accelerator designs givne the varying parallelism strategies across stages (see below for details). 

